Bitcoin Coin Selection with Leverage

We present a new Bitcoin coin selection algorithm, "coin selection with leverage", which aims to improve upon cost savings than that of standard knapsack like approaches. Parameters to the new algorithm are available to be tuned at the users discretion to address other goals of coin selection. Our approach naturally fits as a replacement for the standard knapsack ingredient of full coin selection procedures.

==> at_scale1.tex <==
\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
  
  %%%% old table - has errors
  
  
    \begin{tabular}{llrrll}
    \toprule
       &    &  \% Savings Per&  Savings Per &    Savings Per Day &     Savings Per Month \\
    $\gamma$ & $M$ &          Payment Request                  &   Payment Request                       &                    &                       \\
    \midrule
    22 & 2  &                   2.161472 &                 0.005293 &  \$158.8 -  \$211.73 &   \$4,763.9 -  \$6,351.87 \\
       & 3  &                   1.708508 &                 0.003156 &  \$94.68 -  \$126.24 &  \$2,840.39 -  \$3,787.19 \\
       & 5  &                   1.530141 &                 0.002092 &   \$62.75 -  \$83.66 &  \$1,882.45 -  \$2,509.94 \\
       & 10 &                   0.655868 &                 0.000659 &   \$19.76 -  \$26.35 &     \$592.9 -  \$790.53 \\
    \bottomrule
    \end{tabular}}
    \caption{A glance at savings approximating market conditions from October 2019 with one BTC = $\$8,582$ and $\gamma = 22$.}
    \label{at_scale1}
\end{table}



==> at_scale2.tex <==

%%% Old Table - has errors

\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llrrll}
    \toprule
       &    &  \% Savings Per&  Savings Per &    Savings Per Day &     Savings Per Month \\
    \gamma & $M$ &          Payment Request                  &   Payment Request                       &                    &                       \\
    \midrule
    900 & 2  &                   0.563130 &                 0.418501 &  \$12,555.03 - \$16,740.05 &   \$376,651.04 - \$502,201.38 \\
        & 3  &                   1.637678 &                 0.953068 &  \$28,592.05 -  \$38,122.73 &  \$857,761.41 -  \$1,143,681.88 \\
        & 5  &                   1.272223 &                 0.560110 &    \$16,803.3 -  \$22,404.4 &   \$504,098.92 -  \$672,131.89 \\
        & 10 &                   1.198339 &                 0.392375 &  \$11,771.26 -  \$15,695.01 &   \$353,137.68 -  \$470,850.24 \\
    \bottomrule
    \end{tabular}}
    \caption{A glance at savings approximating market conditions from January 2018 with one BTC = $\$17,174$ and $\gamma = 900$.}
    \label{tab:my_label}
\end{table}





==> table_test.tex <==
\begin{tabular}{rrrrr}
\toprule
 Iterations &  boostFactor &  costPerPayRequest &  executionTime &  feePerByte \\
\midrule
          5 &         0.94 &           0.239808 &      46.012276 &          22 \\
          5 &         0.94 &           0.238512 &      44.234029 &          22 \\
          5 &         0.94 &           0.239543 &      57.311989 &          22 \\
          5 &         0.94 &           0.240052 &      45.827778 &          22 \\
          5 &         0.94 &           0.238879 &      51.464904 &          22 \\
\bottomrule
\end{tabular}


==> test2.tex <==
\begin{tabular}{llrrrrrr}
\toprule
    &    &  Fallback Success Rate &  numKnapsackSolns &  Leverage Success Rate &  numPayRequestsProcessed &  Cost Per Pay Request (one BTC = \$8,582) &  Cost Per Pay Request (one BTC = \$17,174) \\
feePerByte & numPayRequestsPerTX &                        &                   &                        &                          &                                          &                                           \\
\midrule
22  & 2  &                   0.94 &              0.06 &                    0.0 &                      100 &                                 0.244890 &                                  0.490065 \\
    & 3  &                   0.96 &              0.04 &                    0.0 &                      150 &                                 0.184722 &                                  0.369660 \\
    & 5  &                   1.00 &              0.00 &                    0.0 &                      250 &                                 0.136694 &                                  0.273547 \\
    & 10 &                   1.00 &              0.00 &                    0.0 &                      500 &                                 0.100444 &                                  0.201004 \\
60  & 2  &                   0.78 &              0.22 &                    0.0 &                      100 &                                 0.657344 &                                  1.315453 \\
    & 3  &                   0.96 &              0.04 &                    0.0 &                      150 &                                 0.503280 &                                  1.007147 \\
    & 5  &                   0.94 &              0.06 &                    0.0 &                      250 &                                 0.372113 &                                  0.744660 \\
    & 10 &                   0.98 &              0.02 &                    0.0 &                      500 &                                 0.273701 &                                  0.547720 \\
200 & 2  &                   0.54 &              0.46 &                    0.0 &                      100 &                                 2.159708 &                                  4.321933 \\
    & 3  &                   0.64 &              0.36 &                    0.0 &                      150 &                                 1.645127 &                                  3.292172 \\
    & 5  &                   0.84 &              0.16 &                    0.0 &                      250 &                                 1.232979 &                                  2.467395 \\
    & 10 &                   0.96 &              0.04 &                    0.0 &                      500 &                                 0.911609 &                                  1.824280 \\
400 & 2  &                   0.52 &              0.48 &                    0.0 &                      100 &                                 4.281211 &                                  8.567411 \\
    & 3  &                   0.52 &              0.48 &                    0.0 &                      150 &                                 3.244493 &                                  6.492767 \\
    & 5  &                   0.66 &              0.34 &                    0.0 &                      250 &                                 2.441034 &                                  4.884913 \\
    & 10 &                   0.86 &              0.14 &                    0.0 &                      500 &                                 1.818567 &                                  3.639253 \\
900 & 2  &                   0.22 &              0.78 &                    0.0 &                      100 &                                 9.273401 &                                 18.557607 \\
    & 3  &                   0.44 &              0.56 &                    0.0 &                      150 &                                 7.261839 &                                 14.532140 \\
    & 5  &                   0.64 &              0.36 &                    0.0 &                      250 &                                 5.493654 &                                 10.993708 \\
    & 10 &                   0.82 &              0.18 &                    0.0 &                      500 &                                 4.085761 &                                  8.176283 \\
\bottomrule
\end{tabular}

